Scattering of two and three physical pions at maximal isospin from lattice QCD

We present the first direct $N_f=2$ lattice QCD computation of two- and three-$\pi^+$ scattering quantities that includes an ensemble at the physical point. We study the quark mass dependence of the two-pion phase shift, and the three-particle interaction parameters. We also compare to phenomenology and chiral perturbation theory (ChPT). In the two-particle sector, we observe good agreement to the phenomenological fits in $s$- and $d$-wave, and obtain $M_\pi a_0 = -0.0481(86)$ at the physical point from a direct computation. In the three-particle sector, we observe reasonable agreement at threshold to the leading order chiral expansion, i.e.\@ a mildly attractive three-particle contact term. In contrast, we observe that the energy-dependent part of the three-particle quasilocal scattering quantity is not well described by leading order ChPT.

==> plots/cm_mass_1_with_threshold.tex <==
% Created by tikzDevice version 0.12.3 on 2020-09-03 08:30:12
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (238.49,505.89);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (238.49,505.89);
\end{scope}
\begin{scope}
\path[clip] ( 27.31, 40.19) rectangle (232.99,500.39);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 27.31, 40.19) rectangle (232.99,500.39);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,134.80) --
	(232.99,134.80);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,280.21) --
	(232.99,280.21);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,425.62) --
	(232.99,425.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31, 62.10) --
	(232.99, 62.10);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,207.51) --
	(232.99,207.51);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,352.91) --
	(232.99,352.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,498.32) --
	(232.99,498.32);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36, 40.19) --
	( 42.36,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45, 40.19) --
	( 67.45,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.53, 40.19) --
	( 92.53,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61, 40.19) --
	(117.61,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69, 40.19) --
	(142.69,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.78, 40.19) --
	(167.78,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86, 40.19) --
	(192.86,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (217.94, 40.19) --
	(217.94,500.39);
\definecolor{drawColor}{gray}{0.40}

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,207.51) -- (232.99,207.51);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,352.91) -- (232.99,352.91);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,479.47) -- (232.99,479.47);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 29.82,197.72) {$4 \pi$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 29.82,343.13) {$6 \pi$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 29.82,469.69) {$2\pi + \rho$};
\definecolor{drawColor}{gray}{0.40}

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 81.24,104.41) --
	(103.82,104.41);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 92.53,104.41) --
	( 92.53,104.41);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 81.24,104.41) --
	(103.82,104.41);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (106.32,126.01) --
	(128.90,126.01);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (117.61,126.01) --
	(117.61,126.01);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (106.32,126.01) --
	(128.90,126.01);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (106.32,177.69) --
	(128.90,177.69);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (117.61,177.69) --
	(117.61,177.69);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (106.32,177.69) --
	(128.90,177.69);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.41,141.62) --
	(153.98,141.62);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (142.69,141.62) --
	(142.69,141.62);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.41,141.62) --
	(153.98,141.62);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.41,213.56) --
	(153.98,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (142.69,213.56) --
	(142.69,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.41,213.56) --
	(153.98,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57, 62.10) --
	(204.15, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (192.86, 62.10) --
	(192.86, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57, 62.10) --
	(204.15, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57,154.13) --
	(204.15,154.13);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (192.86,154.13) --
	(192.86,154.13);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57,154.13) --
	(204.15,154.13);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57,255.96) --
	(204.15,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (192.86,255.96) --
	(192.86,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (181.57,255.96) --
	(204.15,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 31.08, 62.10) --
	( 53.65, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 42.36, 62.10) --
	( 42.36, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 31.08, 62.10) --
	( 53.65, 62.10);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 31.08,255.96) --
	( 53.65,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 42.36,255.96) --
	( 42.36,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 31.08,255.96) --
	( 53.65,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (206.65,255.96) --
	(229.23,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (217.94,255.96) --
	(217.94,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (206.65,255.96) --
	(229.23,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (156.49,213.56) --
	(179.06,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (167.78,213.56) --
	(167.78,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (156.49,213.56) --
	(179.06,213.56);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 56.16,255.96) --
	( 78.73,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 67.45,255.96) --
	( 67.45,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 56.16,255.96) --
	( 78.73,255.96);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 56.16,373.92) --
	( 78.73,373.92);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 67.45,373.92) --
	( 67.45,373.92);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 56.16,373.92) --
	( 78.73,373.92);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 81.24,109.00) --
	(103.82,109.00);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.53,109.00) --
	( 92.53,109.00);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 81.24,109.00) --
	(103.82,109.00);

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.32,130.74) --
	(128.90,130.74);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61,130.74) --
	(117.61,130.74);

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.32,130.74) --
	(128.90,130.74);

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.32,182.31) --
	(128.90,182.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61,182.31) --
	(117.61,182.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (106.32,182.31) --
	(128.90,182.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.41,146.45) --
	(153.98,146.45);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69,146.45) --
	(142.69,146.45);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.41,146.45) --
	(153.98,146.45);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.41,226.99) --
	(153.98,226.99);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69,226.99) --
	(142.69,226.99);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.41,226.99) --
	(153.98,226.99);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57, 62.84) --
	(204.15, 62.84);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86, 62.84) --
	(192.86, 62.84);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57, 62.84) --
	(204.15, 62.84);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57,159.49) --
	(204.15,159.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86,159.49) --
	(192.86,159.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57,159.49) --
	(204.15,159.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57,262.89) --
	(204.15,262.89);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86,262.89) --
	(192.86,262.89);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.57,262.89) --
	(204.15,262.89);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.08, 63.90) --
	( 53.65, 63.90);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36, 63.90) --
	( 42.36, 63.90);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.08, 63.90) --
	( 53.65, 63.90);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.08,270.08) --
	( 53.65,270.08);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36,270.08) --
	( 42.36,270.08);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.08,270.08) --
	( 53.65,270.08);

\path[draw=drawColor,line width= 0.6pt,line join=round] (206.65,257.88) --
	(229.23,257.88);

\path[draw=drawColor,line width= 0.6pt,line join=round] (217.94,257.88) --
	(217.94,257.88);

\path[draw=drawColor,line width= 0.6pt,line join=round] (206.65,257.88) --
	(229.23,257.88);

\path[draw=drawColor,line width= 0.6pt,line join=round] (156.49,214.59) --
	(179.06,214.59);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.78,214.59) --
	(167.78,214.59);

\path[draw=drawColor,line width= 0.6pt,line join=round] (156.49,214.59) --
	(179.06,214.59);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 56.16,258.52) --
	( 78.73,258.52);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45,258.52) --
	( 67.45,258.52);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 56.16,258.52) --
	( 78.73,258.52);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 56.16,377.97) --
	( 78.73,377.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45,377.97) --
	( 67.45,377.97);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 56.16,377.97) --
	( 78.73,377.97);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36, 63.65) -- ( 42.36, 64.64);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36,267.42) -- ( 42.36,271.45);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45,257.45) -- ( 67.45,260.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45,371.42) -- ( 67.45,378.92);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.53,106.69) -- ( 92.53,108.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61,129.36) -- (117.61,132.56);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61,181.75) -- (117.61,186.06);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69,140.05) -- (142.69,149.38);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69,223.27) -- (142.69,234.59);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.78,202.19) -- (167.78,212.79);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86, 61.11) -- (192.86, 71.45);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86,168.02) -- (192.86,178.07);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86,258.83) -- (192.86,271.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (217.94,264.60) -- (217.94,275.62);
\definecolor{fillColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 42.36, 64.15) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 42.36,269.43) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 67.45,259.18) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 67.45,375.17) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 92.53,107.80) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (117.61,130.96) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (117.61,183.90) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (142.69,144.71) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (142.69,228.93) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (167.78,207.49) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (192.86, 66.28) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (192.86,173.05) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (192.86,264.94) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (217.94,270.11) circle (  1.25);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 27.31, 40.19) rectangle (232.99,500.39);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36, 59.07) {2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,204.48) {4};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,349.88) {6};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,495.29) {8};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56, 62.10) --
	( 27.31, 62.10);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,207.51) --
	( 27.31,207.51);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,352.91) --
	( 27.31,352.91);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,498.32) --
	( 27.31,498.32);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 42.36, 37.44) --
	( 42.36, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 67.45, 37.44) --
	( 67.45, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 92.53, 37.44) --
	( 92.53, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.61, 37.44) --
	(117.61, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (142.69, 37.44) --
	(142.69, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.78, 37.44) --
	(167.78, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (192.86, 37.44) --
	(192.86, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (217.94, 37.44) --
	(217.94, 40.19);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 42.36, 29.18) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 42.36, 19.68) {$\mathrm A_1^+$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 67.45, 29.18) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 67.45, 19.68) {$\mathrm E^+$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 92.53, 29.18) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 92.53, 19.68) {$\mathrm A_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (117.61, 29.18) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (117.61, 19.68) {$\mathrm A_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (142.69, 29.18) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (142.69, 19.68) {$\mathrm A_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (167.78, 29.18) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (167.78, 19.68) {$\mathrm E$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (192.86, 29.18) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (192.86, 19.68) {$\mathrm A_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (217.94, 29.18) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (217.94, 19.68) {$\mathrm B_1$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (130.15,  7.64) {$\vec P^2, \Gamma$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,270.29) {$a E / a M_\pi$};
\end{scope}
\end{tikzpicture}


==> plots/cm_mass_2_with_threshold.tex <==
% Created by tikzDevice version 0.12.3 on 2020-09-03 08:30:21
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (238.49,505.89);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (238.49,505.89);
\end{scope}
\begin{scope}
\path[clip] ( 27.31, 40.19) rectangle (232.99,500.39);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 27.31, 40.19) rectangle (232.99,500.39);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31, 97.55) --
	(232.99, 97.55);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,170.42) --
	(232.99,170.42);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,243.30) --
	(232.99,243.30);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,316.17) --
	(232.99,316.17);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,389.05) --
	(232.99,389.05);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 27.31,461.93) --
	(232.99,461.93);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31, 61.11) --
	(232.99, 61.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,133.98) --
	(232.99,133.98);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,206.86) --
	(232.99,206.86);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,279.74) --
	(232.99,279.74);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,352.61) --
	(232.99,352.61);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,425.49) --
	(232.99,425.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 27.31,498.37) --
	(232.99,498.37);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22, 40.19) --
	( 47.22,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.39, 40.19) --
	( 80.39,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (113.57, 40.19) --
	(113.57,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74, 40.19) --
	(146.74,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (179.91, 40.19) --
	(179.91,500.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09, 40.19) --
	(213.09,500.39);
\definecolor{drawColor}{gray}{0.40}

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,206.86) -- (232.99,206.86);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,352.61) -- (232.99,352.61);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 1pt off 3pt ,line join=round] ( 27.31,479.47) -- (232.99,479.47);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 30.63,197.07) {$5 \pi$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 30.63,342.82) {$7 \pi$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 30.63,469.68) {$3\pi + \rho$};
\definecolor{drawColor}{gray}{0.40}

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 32.29, 61.11) --
	( 62.15, 61.11);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 47.22, 61.11) --
	( 47.22, 61.11);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 32.29, 61.11) --
	( 62.15, 61.11);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 32.29,255.43) --
	( 62.15,255.43);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 47.22,255.43) --
	( 47.22,255.43);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 32.29,255.43) --
	( 62.15,255.43);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 98.64,118.38) --
	(128.49,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (113.57,118.38) --
	(113.57,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 98.64,118.38) --
	(128.49,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.81,148.02) --
	(161.67,148.02);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (146.74,148.02) --
	(146.74,148.02);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.81,148.02) --
	(161.67,148.02);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.81,193.65) --
	(161.67,193.65);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (146.74,193.65) --
	(146.74,193.65);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (131.81,193.65) --
	(161.67,193.65);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (164.98,169.55) --
	(194.84,169.55);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (179.91,169.55) --
	(179.91,169.55);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (164.98,169.55) --
	(194.84,169.55);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (198.16,118.38) --
	(228.01,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (213.09,118.38) --
	(213.09,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (198.16,118.38) --
	(228.01,118.38);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (198.16,186.87) --
	(228.01,186.87);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (213.09,186.87) --
	(213.09,186.87);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] (198.16,186.87) --
	(228.01,186.87);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 65.46,255.43) --
	( 95.32,255.43);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 80.39,255.43) --
	( 80.39,255.43);

\path[draw=drawColor,line width= 0.6pt,dash pattern=on 4pt off 4pt ,line join=round] ( 65.46,255.43) --
	( 95.32,255.43);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.29, 66.94) --
	( 62.15, 66.94);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22, 66.94) --
	( 47.22, 66.94);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.29, 66.94) --
	( 62.15, 66.94);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.29,282.25) --
	( 62.15,282.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22,282.25) --
	( 47.22,282.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.29,282.25) --
	( 62.15,282.25);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.64,130.13) --
	(128.49,130.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (113.57,130.13) --
	(113.57,130.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.64,130.13) --
	(128.49,130.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.81,159.58) --
	(161.67,159.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74,159.58) --
	(146.74,159.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.81,159.58) --
	(161.67,159.58);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.81,209.11) --
	(161.67,209.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74,209.11) --
	(146.74,209.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] (131.81,209.11) --
	(161.67,209.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] (164.98,181.07) --
	(194.84,181.07);

\path[draw=drawColor,line width= 0.6pt,line join=round] (179.91,181.07) --
	(179.91,181.07);

\path[draw=drawColor,line width= 0.6pt,line join=round] (164.98,181.07) --
	(194.84,181.07);

\path[draw=drawColor,line width= 0.6pt,line join=round] (198.16,130.41) --
	(228.01,130.41);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09,130.41) --
	(213.09,130.41);

\path[draw=drawColor,line width= 0.6pt,line join=round] (198.16,130.41) --
	(228.01,130.41);

\path[draw=drawColor,line width= 0.6pt,line join=round] (198.16,199.63) --
	(228.01,199.63);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09,199.63) --
	(213.09,199.63);

\path[draw=drawColor,line width= 0.6pt,line join=round] (198.16,199.63) --
	(228.01,199.63);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 65.46,263.16) --
	( 95.32,263.16);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.39,263.16) --
	( 80.39,263.16);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 65.46,263.16) --
	( 95.32,263.16);
\definecolor{drawColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22, 65.17) -- ( 47.22, 70.96);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22,273.88) -- ( 47.22,292.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.39,263.53) -- ( 80.39,283.92);

\path[draw=drawColor,line width= 0.6pt,line join=round] (113.57,122.94) -- (113.57,133.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74,155.60) -- (146.74,166.39);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74,203.08) -- (146.74,209.81);

\path[draw=drawColor,line width= 0.6pt,line join=round] (179.91,178.45) -- (179.91,189.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09,122.50) -- (213.09,133.65);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09,213.34) -- (213.09,232.16);
\definecolor{fillColor}{RGB}{255,0,0}

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 47.22, 68.06) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 47.22,283.18) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] ( 80.39,273.72) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (113.57,128.03) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (146.74,160.99) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (146.74,206.44) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (179.91,184.03) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (213.09,128.07) circle (  1.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round,fill=fillColor] (213.09,222.75) circle (  1.25);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 27.31, 40.19) rectangle (232.99,500.39);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36, 58.08) {3};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,130.95) {4};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,203.83) {5};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,276.71) {6};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,349.58) {7};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,422.46) {8};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 22.36,495.34) {9};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56, 61.11) --
	( 27.31, 61.11);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,133.98) --
	( 27.31,133.98);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,206.86) --
	( 27.31,206.86);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,279.74) --
	( 27.31,279.74);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,352.61) --
	( 27.31,352.61);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,425.49) --
	( 27.31,425.49);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 24.56,498.37) --
	( 27.31,498.37);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 47.22, 37.44) --
	( 47.22, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 80.39, 37.44) --
	( 80.39, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (113.57, 37.44) --
	(113.57, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (146.74, 37.44) --
	(146.74, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (179.91, 37.44) --
	(179.91, 40.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (213.09, 37.44) --
	(213.09, 40.19);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 47.22, 29.18) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 47.22, 19.68) {$\mathrm A_1^-$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 80.39, 29.18) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 80.39, 19.68) {$\mathrm E^-$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (113.57, 29.18) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (113.57, 19.68) {$\mathrm A_2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (146.74, 29.18) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (146.74, 19.68) {$\mathrm A_2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (179.91, 29.18) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (179.91, 19.68) {$\mathrm A_2$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (213.09, 29.18) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (213.09, 19.68) {$\mathrm A_2$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (130.15,  7.64) {$\vec P^2, \Gamma$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (238.49,505.89);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 13.08,270.29) {$a E / a M_\pi$};
\end{scope}
\end{tikzpicture}

